Position paper: A systematic framework for categorising IoT device fingerprinting mechanisms

The popularity of the Internet of Things (IoT) devices makes it increasingly important to be able to fingerprint them, for example in order to detect if there are misbehaving or even malicious IoT devices in one's network. The aim of this paper is to provide a systematic categorisation of machine learning augmented techniques that can be used for fingerprinting IoT devices. This can serve as a baseline for comparing various IoT fingerprinting mechanisms, so that network administrators can choose one or more mechanisms that are appropriate for monitoring and maintaining their network. We carried out an extensive literature review of existing papers on fingerprinting IoT devices -- paying close attention to those with machine learning features. This is followed by an extraction of important and comparable features among the mechanisms outlined in those papers. As a result, we came up with a key set of terminologies that are relevant both in the fingerprinting context and in the IoT domain. This enabled us to construct a framework called IDWork, which can be used for categorising existing IoT fingerprinting mechanisms in a way that will facilitate a coherent and fair comparison of these mechanisms. We found that the majority of the IoT fingerprinting mechanisms take a passive approach -- mainly through network sniffing -- instead of being intrusive and interactive with the device of interest. Additionally, a significant number of the surveyed mechanisms employ both static and dynamic approaches, in order to benefit from complementary features that can be more robust against certain attacks such as spoofing and replay attacks.

==> hardware.tex <==
\begin {figure*}%[!hbtp]
\centering
\begin{adjustbox}{width=0.9\textwidth}
\begin{tikzpicture}[ every node/.style = {shape=rectangle, rounded corners,draw, align=center, top color=white, bottom color=gray!45}, level 1/.style={sibling distance=140mm},level 2/.style={sibling distance=68mm}, level 3/.style={sibling distance=33mm}, level 4/.style={sibling distance=16mm}, level 5/.style={sibling distance=7mm}, level 5/.style={sibling distance=5mm}]
    \node {H/W Feature} 
        child{ node {Active}
            child{ node {Static}
                child{ node {F/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{\textbf{1}}} %node1
                            }
                        child{ node {C}
                            child{ node{\textbf{2}}} %node 2
                            }
                        child{ node {U}
                            child{ node{\textbf{3}}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{\textbf{4}}}
                            }
                        child{ node {C}
                            child{ node{\textbf{5}}}
                            }
                        child{ node {U}
                            child{ node{\textbf{6}}}
                            }
                        }
                    }%end of F/W
                child{ node {H/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{\textbf{7}}}
                            }
                        child{ node {C}
                            child{ node{\textbf{8}}}
                            }
                        child{ node {U}
                            child{ node{\textbf{9}}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{\textbf{10}}}
                            }
                        child{ node {C}
                            child{ node{\textbf{11}}}
                            }
                        child{ node {U}
                            child{ node{\textbf{12}}}
                            }
                        }
                    }%end of H/W
                } %end of static
            child{ node {Dynamic}
                child{ node {F/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{\textbf{13}}}
                            }
                        child{ node {C}
                            child{ node{\textbf{14}}}
                            }
                        child{ node {U}
                            child{ node{\textbf{15}}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{\textbf{16}}}
                            }
                        child{ node {C}
                            child{ node{\textbf{17}}}
                            }
                        child{ node {U}
                            child{ node{\textbf{18}}}
                            }
                        }
                    }%end of F/W
                child{ node {H/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{\textbf{19}}}
                            }
                        child{ node {C}
                            child{ node{20}}
                            }
                        child{ node {U}
                            child{ node{21}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{22}}
                            }
                        child{ node {C}
                            child{ node{23}}
                            }
                        child{ node {U}
                            child{ node{24}}
                            }
                        }
                    }%end of H/W
                } %end of Dynamic
            }%end of Active   
        child{ node {Passive}
            child{ node {Static}
                child{ node {F/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{25}}
                            }
                        child{ node {C}
                            child{ node{26}}
                            }
                        child{ node {U}
                            child{ node{27}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{28}}
                            }
                        child{ node {C}
                            child{ node{29}}
                            }
                        child{ node {U}
                            child{ node{30}}
                            }
                        }
                    }%end of F/W
                child{ node {H/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{31}}
                            }
                        child{ node {C}
                            child{ node{32}}
                            }
                        child{ node {U}
                            child{ node{33}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{34}}
                            }
                        child{ node {C}
                            child{ node{35}}
                            }
                        child{ node {U}
                            child{ node{36}}
                            }
                        }
                    }%end of H/W
                } %end of static
            child{ node {Dynamic}
                child{ node {F/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{37}}
                            }
                        child{ node {C}
                            child{ node{38}}
                            }
                        child{ node {U}
                            child{ node{39}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{40}}
                            }
                        child{ node {C}
                            child{ node{41}}
                            }
                        child{ node {U}
                            child{ node {42}}
                            }
                        }
                    }%end of F/W
                child{ node {H/W}
                    child{ node {S}
                        child{ node {T}
                            child{ node{43}}
                            }
                        child{ node {C}
                            child{ node{44}}
                            }
                        child{ node {U}
                            child{ node{45}}
                            }
                        }
                    child{ node {ML}
                        child{ node {T}
                            child{ node{46}}
                            }
                        child{ node {C}
                            child{ node{47}}
                            }
                        child{ node {U}
                            child{ node{48}}
                            }
                        }
                    }%end of H/W
                } %end of Dynamic
            };%end of Passive       
\end{tikzpicture}
\end{adjustbox}
\caption{The tree shows the five main  categorisation features arrangement by \system. Abbreviations used in  the tree are S for statistical, H/W for hardware, F/W for firmware,  ML for Machine Learning, T for Type, C for Class, U for  Unique}
\end{figure*}


        

==> htable.tex <==
\begin{table}[]
\caption{The classification of existing IoT fingerprinting mechanisms with ML techniques}
\label{tab:classification}
\begin{tabular}{l|llllll}
 &  &  &  &  &  &  \\
 \hline
 \hline
1 &active  & static & Firmware & Statistical &Type &   \\
\hline
2 & active  & static  &Firmware  & Statistical  & Class &  \\
\hline
3 &active   & static  & Firmware & Statistical & Unique &  \\
\hline
4 & active   & static  & Firmware & ML & Type  &  \\
\hline
5 & active  &  static & Firmware & ML & Class &  \\
\hline
6 & active  &  static & Firmware &  ML & Unique &  \\
\hline
7 & active  & static  & Hardware & Statistical & Type &  \\
\hline
8 & active  & static  &  Hardware & Statistical  &Class  &  \\
\hline
9 & active  & static  &  Hardware & Statistical & Unique &  \\
\hline
10 &active   & static  &   Hardware&  ML & Type  &  \\
\hline
11 &active   &  static &  Hardware &  ML & Class  &  \\
\hline
12 & active  & static  &  Hardware &  ML & Unique &  \\
\hline
13 & active  & dynamic & Firmware & Statistical &Type  &  \\
\hline
14 & active  & dynamic & Firmware & Statistical & Class &  \\
\hline
15 & active  & dynamic & Firmware & Statistical & Unique &  \\
\hline
16 & active  & dynamic & Firmware & ML  & Type &  \\
\hline
17 & active  & dynamic & Firmware &  ML & Class &  \\
\hline
18 & active  & dynamic & Firmware &  ML & Unique &  \\
\hline
19 & active  & dynamic &  Hardware& Statistical &Type  &  \\
\hline
20 & active  & dynamic & Hardware & Statistical & Class &  \\
\hline 
21 & active  & dynamic & Hardware &Statistical & Unique &  \\
\hline
22 & active  & dynamic & Hardware &  ML & Type &  \\
\hline
23 & active  & dynamic & Hardware &  ML & Class &  \\
\hline
24 & active  & dynamic &  Hardware & ML  & Unique &  \\
\hline
25 & passive  & static & Firmware  &Statistical  & Type &  \\
\hline
26 & passive & static  & Firmware & Statistical & Class  &  \\
\hline
27 & passive & static  &Firmware  & Statistical & Unique  &  \\
\hline
28 & passive & static  & Firmware & ML  & Type &  \\
\hline
29 & passive & static  &Firmware  &  ML & Class &  \\
\hline
30 & passive & static  &Firmware  &  ML & Unique &  \\
\hline
31 & passive & static  &  Hardware & Statistical & Type &  \\
\hline
32 & passive & static  &  Hardware & Statistical & Class &  \\
\hline
33 & passive & static  &  Hardware & Statistical & Unique &  \\
\hline
34 & passive & static  &  Hardware & ML  & Type  &  \\
\hline
35 & passive & static  &  Hardware &  ML & Class  &  \\
\hline
36 & passive & static &  Hardware &  ML & Unique  &  \\
\hline
37 & passive & dynamic & Firmware & Statistical &Type  &  \\
\hline
38 & passive & dynamic & Firmware & Statistical & Class &  \\
\hline
39 & passive & dynamics  & Firmware & Statistical & Unique &  \\
\hline
40 & passive & dynamic & Firmware & ML  & Type &  \\
\hline
41 & passive & dynamic & Firmware &  ML & Class &  \\
\hline
42 & passive & dynamic & Firmware &  ML & Unique &  \\
\hline
43 & passive & dynamic &  Hardware & Statistical & Type &  \\
\hline
44 & passive & dynamic & Hardware  & Statistical & Class &  \\
\hline
45 & passive & dynamic &  Hardware & Statistical & Unique &  \\
\hline
46 & passive & dynamic &  Hardware &  ML & Type &  \\
\hline
47 & passive & dynamic &  Hardware &  ML & Class &  \\
\hline
48 &  passive& dynamic &  Hardware &  ML & Unique & \\
\hline
\end{tabular}
\end{table}

==> software.tex <==
\begin {figure*}%[!hbtp]
\centering
\begin{adjustbox}{width=\textwidth}
%BA: I added "rotate=90,transform shape" in the tikzpicture parameter to rotate it 90 degrees -- cancelled.
\begin{tikzpicture}[ every node/.style = {shape=rectangle, rounded corners,draw, align=center, top color=white, bottom color=gray!45}, level 1/.style={sibling distance=1mm},level 2/.style={sibling distance=5mm}, level 3/.style={sibling distance=220mm}, level 4/.style={sibling distance=72mm}, level 5/.style={sibling distance=34mm}, level 6/.style={sibling distance=16mm}, level 7/.style={sibling distance=5mm}]
    \node {S/W Feature} 
        child{ node {Active/Passive}
            child{ node {Static/Dynamic}
                child{ node {App}
                    child {node {Packet}
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                     }%end of packet
                    child {node {DF}
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                    }%end of DF 
                    child {node {F} %start of F (BA)
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                    }%end of F (BA)
                }%end of App
                child{ node {Net}
                    child {node {Packet}
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                     }%end of packet
                    child {node {DF}
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                    }%end of DF
                    child {node {F} %start of F (BA)
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                    }%end of F (BA)
                }%end of Net
                child{ node {Mac}
                    child {node {Packet}
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node S
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node S
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                     }%end of packet
                    child {node {DF}
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node S
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node S
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                    }%end of DF
                    child {node {F} %start of F (BA)
                        child {node {H}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of H
                     child {node {P}
                            child{ node {RB}
                                child{ node {T}
                                    }
                                    child{ node {C}
                                    }
                                    child{ node {U}
                                    }
                                }%end of node RB
                            child{ node {ML}
                                child{ node {T}
                                    }
                                child{ node {C}
                                }
                                child{ node {U}
                                }
                                }
                        }%end of P
                    }%end of F (BA)
                }%end of Mac
            }%end of static
        }; %end of active/passive
\end{tikzpicture}
\end{adjustbox}
\caption{The tree shows the seven main  categorisation features arrangement by \system. Abbreviations used in  the tree are Passive/Dynamic, Static/Dynamic, MAC/Network/Application, Packet/Data Frame/Header, Header/Payload, Rule Based/ Machine Learning,  Type/Class/Unique}
\label{tree-sw}
\end{figure*}


